Simulation Environment for Link Energy Estimation in Networks-on-Chip with Virtual Channels

Network-on-chip (NoC) is the most promising design paradigm for the interconnect architecture of a multiprocessor system-on-chip (MPSoC). On the downside, a NoC has a significant impact on the overall energy consumption of the system. NoC simulators are highly relevant for design space exploration even at an early stage. Since links in NoC consume up to 50% of the energy, a realistic energy consumption of links in NoC simulators is important. This work presents a simulation environment which implements a technique to precisely estimate the data dependent link energy consumption in NoCs with virtual channels for the first time. Our model works at a high level of abstraction, making it feasible to estimate the energy requirements at an early design stage. Additionally, it enables the fast evaluation and early exploration of low-power coding techniques. The presented model is applicable for 2D and 3D NoCs. A case study for an image processing application shows that the current link model leads to an underestimate of the link energy consumption by up to a factor of four. In contrast, the technique presented in this paper estimates the energy quantities precisely with an error below 1% compared to results obtained by precise, but computational extensive, bit-level simulation.

==> chapters/bufferDepth.tex <==

\input{tables/flitPlot}
%\input{tables/packetPlot}
\input{tables/networkPlot}

We use the simulator to assess the influence of buffer depth and number of VCs on the case study. This demonstrates the capabilities of the simulator to measure NoC performance. We simulate the case study for a number of 1 -- 6 VCs and a buffer depth of 5 -- 20 flits. The length of a packet is 10 flits. The average flit latency is shown in Fig.~\ref{fig:flitdelay} and the average packet latency in Fig.~\ref{fig:packetdelay}. As expected, the delay is smaller for a larger number of VCs and a larger buffer depth: For a single VC and a buffer depth of 5 flits, the average flit latency is \unit[496]{ns}; for 6 VCs and 20 flits buffer depth, the flit latency is only \unit[38]{ns}. Naturally, the average packet latency is similar. It is noteworthy, that, for a few VCs, the flit and packet latency for 10 flits is larger than for 11 -- 13 flits. This is a result of the packet length of 10 flits. For light back pressure, as in our example, it is advantageous to store more than one packet in the router. 

==> tikz/effect_mux_1.tex <==
% This file was created by matplotlib2tikz v0.6.15.
\begin{tikzpicture}



\end{tikzpicture}


==> tikz/effect_mux_2.tex <==
% This file was created by matplotlib2tikz v0.6.15.
\begin{tikzpicture}

\begin{axis}[
title={BI Coded Uncorrelated Data},
xlabel={Mux Probability},
ylabel={Coding gain in %},
xmin=0, xmax=1,
ymin=-10, ymax=15,
axis on top,
width=\figurewidth,
height=\figureheight,
tick pos=both,
xmajorgrids,
ymajorgrids,
legend entries={{2D Link},{3D Link}},
legend cell align={left}
]
\addlegendimage{no markers, red}
\addlegendimage{no markers, blue}
\addplot [red, mark=*, mark size=3, mark options={solid,draw=black}]
table {%
0 13.3846547767656
0.1 12.2192810815626
0.2 9.64199679556266
0.3 7.61748858994351
0.4 5.00256548051365
0.5 3.12851877402711
0.6 1.75193468363479
0.7 -1.25973438351297
0.8 -0.880998451971826
0.9 -5.14115424512092
1 -6.7730622425823
};
\addplot [blue, mark=square*, mark size=3, mark options={solid,draw=black}]
table {%
0 13.1212345888638
0.1 11.9581219024437
0.2 9.54703318056063
0.3 7.41106466576225
0.4 4.5499935174231
0.5 3.00249453218394
0.6 1.48240817160563
0.7 -1.7092041746946
0.8 -1.01345197141185
0.9 -5.3235629114069
1 -6.7449284508329
};
\end{axis}

\end{tikzpicture}
